Beyond Jarlskog: 699 invariants for CP violation in SMEFT

As SMEFT is a framework of growing importance to analyze high-energy data, understanding its parameter space is crucial. The latter is commonly split into CP-even and CP-odd parts, but this classification is obscured by the fact that CP violation is actually a collective effect that is best captured by considering flavor-invariant combinations of Lagrangian parameters. First we show that fermion rephasing invariance imposes that several coefficients associated to dimension-six operators can never interfere with operators of dimension $\leq4$ and thus cannot appear in any physical observable at $\order{1/\Lambda^2}$. For those that can, instead, we establish a one-to-one correspondence with CP-odd flavor invariants, all linear with respect to SMEFT coefficients. We explicitly present complete lists of such linear CP-odd invariants, and carefully examine their relationship to CP breaking throughout the parameter space of coefficients of dimension $\leq 4$. Requiring that these invariants all vanish, together with the Jarlskog invariant, the strong-CP phase, and the 6 CP-violating dimension-6 bosonic operators, provides $699(+1+1+6)$ conditions for CP conservation to hold in any observable at leading order, $\cO\(1/\Lambda^2\)$.

==> tikzfeynhand.keys.code.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-FeynHand, Version 1.1.0 of 2019/08/19
% Feynhand Diagrams with TikZ (LaTex manual version)
% Copyright (C) 2019 Max Dohse
% Copyright (C) 2016 Joshua Ellis
%
%
% This LaTeX file and the whole package are free: 
% you can redistribute it and/or modify it under the
% terms of the GNU General Public License as published by the Free Software Foundation, 
% either version 3 of the License, or (at your option) any later version.
%
% This file is a modification of the file tikzfeynman.keys.code.tex
% of the package tikz-feynman (version 1.1.0 of 2016/02/05)
% which is available online at https://ctan.org/pkg/tikz-feynman
% for a list of changes, see the file CHANGES.TXT
%
% available at https://ctan.org/pkg/tikz-feynhand
% The Current Maintainer of this work is Max Dohse.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lengths
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newlength{\feynhanddotsize}
\setlength{\feynhanddotsize}{1.5mm}

\newlength{\feynhandblobsize}
\setlength{\feynhandblobsize}{7.5mm}

\newlength{\feynhandlinesize}
\setlength{\feynhandlinesize}{0.5pt}

\newlength{\feynhandarrowsize}
\setlength{\feynhandarrowsize}{6pt}

\newlength{\feynhandtopsep}
\setlength{\feynhandtopsep}{18\feynhandlinesize}

%% Colors
\newcommand{\feynhandtopsepcolor}{white}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynhand@cs@angle@step{30}
      \def\tikzfeynhand@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynhand@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynhand@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynhand@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynhand@cs@points@per@step,
    switch if less than=1.25*\tikzfeynhand@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynhand@cs@current@angle+\tikzfeynhand@cs@angle@step, 360)}
      \let\tikzfeynhand@cs@current@angle=\pgfmathresult%
    },
  ]{
%    \pgfmathparse{sin(\tikzfeynhand@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \pgfmathparse{sin(\tikzfeynhand@cs@current@angle) * 3 * \feynhandlinesize / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzfeynhandset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynhand/.code={},
  execute at end feynhand/.code={},
  every feynhand/.style={/tikzfeynhand/every feynhand@@/.append style={#1}},
  every feynhand@@/.style={
    /tikzfeynhand/.cd,
    },
  execute at begin feynhand@@/.code={}                     %% Internal version
  execute at end feynhand@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynhand/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynhand/every vertex@@,
  },
  %% DOTS + friends
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=\feynhanddotsize,
    /tikz/line width = \feynhandlinesize,
  },
  every dot/.style={/tikzfeynhand/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynhand/every dot@@,
  },
  every squaredot@@/.style={
    /tikz/shape=rectangle,
  },
  every squaredot/.style={/tikzfeynhand/every squaredot@@/.append style={#1}},
  squaredot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every squaredot@@,
  },
  every ringdot@@/.style={
    /tikz/fill=none,
  },
  every ringdot/.style={/tikzfeynhand/every ringdot@@/.append style={#1}},
  ringdot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every ringdot@@,
  },
  every crossdot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=2\feynhanddotsize,
  },
  every crossdot/.style={/tikzfeynhand/every crossdot@@/.append style={#1}},
  crossdot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every crossdot@@,
  },
  %% BLOBS -------------------------------------------------
    every blob@@/.style={
    /tikz/shape=circle,
    /tikz/draw,
    /tikz/fill,
    /tikz/outer sep={0.5*\the\feynhandlinesize},
    /tikz/inner sep=0pt,
    /tikz/minimum size=\feynhandblobsize,
    /tikz/line width = \feynhandlinesize,
  },
  every blob/.style={/tikzfeynhand/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynhand/every blob@@,
    /tikz/fill=black,
  },
  every ringblob@@/.style={
  },
  every ringblob/.style={/tikzfeynhand/every ringblob@@/.append style={#1}},
  ringblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every ringblob@@,
    /tikz/fill=white,
  },
  every NWblob@@/.style={
  },
  every NWblob/.style={/tikzfeynhand/every NWblob@@/.append style={#1}},
  NWblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every NWblob@@,
    /tikz/fill=none,
    /tikz/pattern=north west lines,
  },
  every NEblob@@/.style={
  },
  every NEblob/.style={/tikzfeynhand/every NEblob@@/.append style={#1}},
  NEblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every NEblob@@,
    /tikz/fill=none,
    /tikz/pattern=north east lines,
  },
  every grayblob@@/.style={
  },
  every grayblob/.style={/tikzfeynhand/every grayblob@@/.append style={#1}},
  grayblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every grayblob@@,
    /tikz/fill=gray!50!white,
  },
  %% PARTICLES
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep={0.5*\the\feynhandlinesize},
  },
  every particle/.style={/tikzfeynhand/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynhand/every particle@@,
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynhand@arrow@size,
  arrow size=\feynhandarrowsize,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          %xshift=0.5mm,
          xshift=-0.166666\feynhandarrowsize,
          fill,
          inner sep=0mm,
          minimum width = \tikzfeynhand@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          %xshift=0.5mm,
          xshift=0.166666\feynhandarrowsize,
          rotate=180,
          fill,
          inner sep=0mm,
          minimum width = \tikzfeynhand@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynhand/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
    },
  },
  every plain/.style={/tikzfeynhand/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynhand/every plain@@,
  },
  every top@@/.style={
    /tikz/preaction={draw=\feynhandtopsepcolor,line width=\feynhandtopsep} 
  },
  every top/.style={/tikzfeynhand/every top@@/.append style={#1}},
  top/.style={
    /tikzfeynhand/every top@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        complete sines,
        amplitude=3\feynhandlinesize,
        segment length=7.5\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynhand/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynhand/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynhand/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynhand/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynhand/boson,
    /tikzfeynhand/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynhand/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynhand/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynhand/boson,
    /tikzfeynhand/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        complete sines,
        amplitude=3\feynhandlinesize,
        segment length=7.5\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynhand/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynhand/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every scalar/.style={/tikzfeynhand/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynhand/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynhand/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynhand/scalar,
    /tikzfeynhand/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynhand/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynhand/scalar,
    /tikzfeynhand/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/line width = 2\feynhandlinesize,
    },
  },
  every ghost/.style={/tikzfeynhand/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynhand/every ghost@@,
  },
  every charged ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every charged ghost/.style={/tikzfeynhand/every charged ghost@@/.append style={#1}},
  charged ghost/.style={
    /tikzfeynhand/ghost,
    /tikzfeynhand/every charged ghost@@,
  },
  every anti charged ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti charged ghost/.style={/tikzfeynhand/every anti charged ghost@@/.append style={#1}},
  anti charged ghost/.style={
    /tikzfeynhand/ghost,
    /tikzfeynhand/every anti charged scalar@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynhand/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynhand/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynhand/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynhand/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynhand/with arrow=0.33,
      /tikzfeynhand/with reversed arrow=0.73,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every majorana/.style={/tikzfeynhand/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynhand/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynhand/with reversed arrow=0.33,
      /tikzfeynhand/with arrow=0.73,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every anti majorana/.style={/tikzfeynhand/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynhand/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        coil,
        aspect=1.2,
        mirror,
        amplitude=3\feynhandlinesize,
        segment length=8\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynhand/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynhand/every gluon@@,
  },
  % short versions of style names
  pho/.style={
    /tikzfeynhand/photon,
  },
  bos/.style={
    /tikzfeynhand/boson,
  },
  antbos/.style={
    /tikzfeynhand/anti charged boson,
  },
  chabos/.style={
    /tikzfeynhand/charged boson,
  },
  sca/.style={
  	/tikzfeynhand/scalar,
  },
  chasca/.style={
  	/tikzfeynhand/charged scalar,
  },
  antsca/.style={
    /tikzfeynhand/anti charged scalar,
  },
  fer/.style={
    /tikzfeynhand/fermion,
  },
  antfer/.style={
    /tikzfeynhand/anti fermion,
  },
  gho/.style={
    /tikzfeynhand/ghost,
  },
  chagho/.style={
    /tikzfeynhand/charged ghost,
  },
  antgho/.style={
    /tikzfeynhand/anti charged ghost,
  },
  glu/.style={
    /tikzfeynhand/gluon,
  },
  maj/.style={
    /tikzfeynhand/majorana,
  },
  antmaj/.style={
    /tikzfeynhand/anti majorana,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynhand@insertion@size,
  insertion/size=5\feynhandlinesize,
  insertion/style/.store in=\tikzfeynhand@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynhandset{insertion/.cd,#1}
        \draw [\tikzfeynhand@insertion@style] (-\tikzfeynhand@insertion@size, -\tikzfeynhand@insertion@size) -- (\tikzfeynhand@insertion@size, \tikzfeynhand@insertion@size);
        \draw [\tikzfeynhand@insertion@style] (-\tikzfeynhand@insertion@size, \tikzfeynhand@insertion@size) -- (\tikzfeynhand@insertion@size, -\tikzfeynhand@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%
  %% Slashes
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  slash/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  slash/size/.store in=\tikzfeynhand@slash@size,
  slash/size=5\feynhandlinesize,
  slash/style/.store in=\tikzfeynhand@slash@style,
  slash/style={},
  %% Styles
  slash@@/.style args={[#1]#2}{
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynhandset{slash/.cd,#1}
        \draw [\tikzfeynhand@slash@style] (-\tikzfeynhand@slash@size, -2*\tikzfeynhand@slash@size) -- (\tikzfeynhand@slash@size, 2*\tikzfeynhand@slash@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  slash@@/.default={[]0.5},
  %%
  %% Backslashes
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  backslash/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  backslash/size/.store in=\tikzfeynhand@backslash@size,
  backslash/size=5\feynhandlinesize,
  backslash/style/.store in=\tikzfeynhand@backslash@style,
  backslash/style={},
  %% Styles
  backslash@@/.style args={[#1]#2}{
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynhandset{backslash/.cd,#1}
        \draw [\tikzfeynhand@backslash@style] (-\tikzfeynhand@backslash@size, 2*\tikzfeynhand@backslash@size) -- (\tikzfeynhand@backslash@size, -2*\tikzfeynhand@backslash@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  backslash@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynhand@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynhand@momentum@arrow@distance,
  momentum/arrow distance={\the\feynhandarrowsize},
  momentum/arrow shorten/.store in=\tikzfeynhand@momentum@arrow@shorten,
  momentum/arrow shorten=0.2,
  momentum/label style/.store in=\tikzfeynhand@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynhand@momentum@arrow@style,
  momentum/arrow style={},
  momentum/arrow thickness/.store in=\tikzfeynhand@momentum@arrow@thickness,
  momentum/arrow thickness={0.64*\the\feynhandlinesize},
  momentum/arrow size/.store in=\tikzfeynhand@momentum@arrow@size,
  momentum/arrow size={0.8*\the\feynhandarrowsize},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
  },
  half right/.style={
    /tikz/bend right=90,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

\endinput

==> tikzlibraryfeynhand.code.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-FeynHand, Version 1.1.0 of 2019/08/19
% Feynhand Diagrams with TikZ (LaTex manual version)
% Copyright (C) 2019 Max Dohse
% Copyright (C) 2016 Joshua Ellis
%
% This LaTeX file and the whole package are free: 
% you can redistribute it and/or modify it under the
% terms of the GNU General Public License as published by the Free Software Foundation, 
% either version 3 of the License, or (at your option) any later version.
%
% This file is a modification of the file tikzlibraryfeynman.code.tex
% of the package tikz-feynman (version 1.1.0 of 2016/02/05)
% which is available online at https://ctan.org/pkg/tikz-feynman
% for a list of changes, see the file CHANGES.TXT
%
% available at https://ctan.org/pkg/tikz-feynhand
% The Current Maintainer of this work is Max Dohse.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Pre-requisites
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
  arrows.meta,
  calc,
  decorations,
  decorations.markings,
  decorations.pathmorphing,
  decorations.pathreplacing,
  external,
  patterns,
  positioning,
  shapes.geometric,
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Miscellaneous functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@empty{}

%% Key Manager
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Setup the tikz-feynhand key family
\pgfkeys{
  /tikzfeynhand/.is family,
  /tikzfeynhand/.search also={/tikz},
}

%% |\tikzfeynhandset| allows keys that belong with tikz-feynhand to be easily set.
\def\tikzfeynhandset{\pgfqkeys{/tikzfeynhand}}

%% Version check
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check which version is expected and which is installed
\def\tikzfeynhand@compat@parse#1.#2.#3\pgfeov{
  \edef\tikzfeynhand@compat@major{#1}
  \edef\tikzfeynhand@compat@minor{#2}
  \edef\tikzfeynhand@compat@patch{#3}
  \edef\tikzfeynhand@compat{#1.#2.#3}
}
\let\tikzfeynhand@compat=\tikzfeynhand@empty
\pgfkeyslet{/tikzfeynhand/compat/.@cmd}{\tikzfeynhand@compat@parse}
\ProcessPgfPackageOptions{/tikzfeynhand}

\AtBeginDocument{
  \ifx\tikzfeynhand@version\tikzfeynhand@compat\else
    \ifx\tikzfeynhand@compat\tikzfeynhand@empty
      \PackageWarning{tikz-feynhand}{Consider loading TikZ-Feynhand with \string\usepackage[compat=\tikzfeynhand@version]{tikz-feynhand} so that you can be warned if TikZ-Feynhand changes.}
    \else
      \ifx\tikzfeynhand@compat@major\tikzfeynhand@version@major
        \ifx\tikzfeynhand@compat@minor\tikzfeynhand@version@minor
          \ifx\tikzfeynhand@compat@patch\tikzfeynhand@version@patch\else
            \PackageInfo{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  This should cause no issue.}
          \fi
        \else
          \PackageWarning{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  This may change some diagrams.}
        \fi
      \else
        \PackageError{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  They are most likely incompatible.  Please download the appropriate version from jpellis.me/projects/tikz-feynhand.}
      \fi
    \fi
  \fi
}

%% Feynhand Environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Provide `\begin{feynhand} ... \end{feynhand}` within TikZ pictures.
\tikzaddtikzonlycommandshortcutlet\feynhand\tikzfeynhand@environment@feynhand
\tikzaddtikzonlycommandshortcutlet\endfeynhand\endtikzfeynhand@environment@feynhand

%% \begin{feynhand}...\end{feynhand}
\def\tikzfeynhand@environment@feynhand{%
  \pgfutil@ifnextchar[{\tikzfeynhand@environment@feynhand@opt}
  {\tikzfeynhand@environment@feynhand@opt[]}}

\def\tikzfeynhand@environment@feynhand@opt[#1]{%
  \begingroup
  %% Local overrides
  \let\tikz@@scan@fig=\tikzfeynhand@scan@fig
  %% Local commands
  \let\vertex=\tikzfeynhand@commands@vertex
  \let\propagator=\tikzfeynhand@commands@propagator
  \let\propag=\propagator
  %% Opening hooks
  \scope
  \tikzfeynhand@tikz@search@tikzfeynhand
  \pgfkeys{/tikzfeynhand/every feynhand@@,#1}
  \pgfkeysvalueof{/tikzfeynhand/execute at begin feynhand@@}%
  \pgfkeysvalueof{/tikzfeynhand/execute at begin feynhand}%
  }

\def\endtikzfeynhand@environment@feynhand{%	
  %% Closing hooks
  \pgfkeysvalueof{/tikzfeynhand/execute at end feynhand}%
  \pgfkeysvalueof{/tikzfeynhand/execute at end feynhand@@}%
  \endscope
  \endgroup
  }

%%% Allow empty nodes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikzfeynhandallowemptynode
\newif\iftikzfeynhandvertex
\def\tikzfeynhand@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
    {\pgfutil@ifnextchar({\tikz@fig@scan@name}
      {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
        {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
          {\iftikzfeynhandvertex%
             \tikzset{/tikzfeynhand/every vertex@@}%
             \iftikzfeynhandallowemptynode%
               \else%
               \tikzset{/tikzfeynhand/particle}%
               \fi%
            \fi%
            \tikz@fig@main{}
          }
        }
      }
    }
}

%% Include /tikzfeynhand in the search path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@tikz@search@tikzfeynhand{%
  \pgfkeys{/tikz/.unknown/.code=%
    \let\tikz@key\pgfkeyscurrentname%
    %% Is it a tikzfeynhand key?
    \pgfkeys{/tikzfeynhand/\tikz@key/.try={##1}}%
    \ifpgfkeyssuccess%
    \else%
      %% Is it a pgf key?
      \pgfkeys{/pgf/\tikz@key/.try={##1}}%
      \ifpgfkeyssuccess%
      \else%
        \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          %% this is a color!
          \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
          \edef\tikz@textcolor{\tikz@key}%
        \else%
          \pgfutil@doifcolorelse{\tikz@key}
          {%
            \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
            \edef\tikz@textcolor{\tikz@key}%
          }%
          {%
            %% Ok, second chance: This might be an arrow specification:
            \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
            \ifpgfutil@in@%
              %% Ah, an arrow spec!
              \expandafter\tikz@processarrows\expandafter{\tikz@key}%
            \else%
              %% Ok, third chance: A shape!
              \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
                \pgfkeys{/errors/unknown key/.expand
                once=\expandafter{\expandafter/\expandafter t\expandafter
                i\expandafter k\expandafter z\expandafter/\tikz@key}{##1}}%
              \else%
                \edef\tikz@shape{\tikz@key}%
              \fi%
            \fi%
          }%
        \fi%
      \fi%
    \fi%
  }
}


%% Vertex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SEE ALSO \vertex above!
%% Adapted from |\coordinate| code
\def\tikzfeynhand@commands@vertex{%
  \path \pgfextra{\tikzfeynhandallowemptynodetrue}
        \pgfextra{\tikzfeynhandvertextrue}
        node}

%% Propagators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tikzfeynhand@commands@propagator}[1][]{\draw [#1]}

%% Optional argument in style key
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@key@opt#1[#2]#3\pgfeov{%
  \tikzfeynhandset{#1={[#2]#3}}}

%% Insertion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@insertion{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{insertion@@}}
  {\tikzfeynhand@key@opt{insertion@@}[]}}
\pgfkeyslet{/tikzfeynhand/insertion/.@cmd}{\tikzfeynhand@insertion}

%% Slash
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@slash{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{slash@@}}
  {\tikzfeynhand@key@opt{slash@@}[]}}
\pgfkeyslet{/tikzfeynhand/slash/.@cmd}{\tikzfeynhand@slash}

%% Backslash
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@backslash{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{backslash@@}}
  {\tikzfeynhand@key@opt{backslash@@}[]}}
\pgfkeyslet{/tikzfeynhand/backslash/.@cmd}{\tikzfeynhand@backslash}

%% Momentum
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@momentum@std{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{momentum@@}}
  {\tikzfeynhand@key@opt{momentum@@}[]}}
\pgfkeyslet{/tikzfeynhand/momentum/.@cmd}{\tikzfeynhand@momentum@std}

\def\tikzfeynhand@momentum@stdp{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{momentum'@@}}
  {\tikzfeynhand@key@opt{momentum'@@}[]}}
\pgfkeyslet{/tikzfeynhand/momentum'/.@cmd}{\tikzfeynhand@momentum@stdp}

\def\tikzfeynhand@momentum@stdr{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{reversed momentum@@}}
  {\tikzfeynhand@key@opt{reversed momentum@@}[]}}
\pgfkeyslet{/tikzfeynhand/reversed momentum/.@cmd}{\tikzfeynhand@momentum@stdr}

\def\tikzfeynhand@momentum@stdrp{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{reversed momentum'@@}}
  {\tikzfeynhand@key@opt{reversed momentum'@@}[]}}
\pgfkeyslet{/tikzfeynhand/reversed momentum'/.@cmd}{\tikzfeynhand@momentum@stdrp}

% short versions of momentum styles
\pgfkeyslet{/tikzfeynhand/rmomentum/.@cmd}{\tikzfeynhand@momentum@stdr}
\pgfkeyslet{/tikzfeynhand/rmomentum'/.@cmd}{\tikzfeynhand@momentum@stdrp}

\pgfkeyslet{/tikzfeynhand/mom/.@cmd}{\tikzfeynhand@momentum@std}
\pgfkeyslet{/tikzfeynhand/mom'/.@cmd}{\tikzfeynhand@momentum@stdp}

\pgfkeyslet{/tikzfeynhand/revmom/.@cmd}{\tikzfeynhand@momentum@stdr}
\pgfkeyslet{/tikzfeynhand/revmom'/.@cmd}{\tikzfeynhand@momentum@stdrp}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input tikzfeynhand.keys.code.tex

\endinput
